PartGlot: Learning Shape Part Segmentation from Language Reference Games

We introduce PartGlot, a neural framework and associated architectures for learning semantic part segmentation of 3D shape geometry, based solely on part referential language. We exploit the fact that linguistic descriptions of a shape can provide priors on the shape's parts -- as natural language has evolved to reflect human perception of the compositional structure of objects, essential to their recognition and use. For training, we use the paired geometry / language data collected in the ShapeGlot work for their reference game, where a speaker creates an utterance to differentiate a target shape from two distractors and the listener has to find the target based on this utterance. Our network is designed to solve this target discrimination problem, carefully incorporating a Transformer-based attention module so that the output attention can precisely highlight the semantic part or parts described in the language. Furthermore, the network operates without any direct supervision on the 3D geometry itself. Surprisingly, we further demonstrate that the learned part information is generalizable to shape classes unseen during training. Our approach opens the possibility of learning 3D shape parts from language alone, without the need for large-scale part geometry annotations, thus facilitating annotation acquisition.

==> rebuttal/rebuttal_body.tex <==
% \newcommand{\ROne}{{\textcolor{red}{\textbf{R1}}}}
% \newcommand{\RTwo}{{\textcolor{Green}{\textbf{R2}}}}
% \newcommand{\RThree}{{\textcolor{blue}{\textbf{R3}}}}
\definecolor{r1}{RGB}{214,39,40}
\definecolor{r2}{RGB}{44,160,44}
\definecolor{r3}{RGB}{31,119,180}
\newcommand{\ROne}{\textbf{\textcolor{r1}{R1}}}
\newcommand{\RTwo}{\textbf{\textcolor{r2}{R2}}}
\newcommand{\RThree}{\textbf{\textcolor{r3}{R3}}}

%%%%%%%
\makeatletter
\definecolor{citecolor}{RGB}{0,255,0}
\newcommand{\citecaron}[1]{[\textcolor{citecolor}{1}]}
\newcommand{\citepartnet}[1]{[\textcolor{citecolor}{2}]}
\makeatother
%%%%%%%


\noindent We thank the reviewers for their valuable comments. Below we answer the specific questions posed. 

\vspace{-\baselineskip}
\paragraph{Paper Novelty and Contributions [\RTwo]} \hfill

%We summarize as follows:

\vspace{-0.5\baselineskip}
\begin{enumerate}[label={(\arabic*)}, itemsep=0em]
    \item We have introduced, for the first time to our knowledge, a method for discovering semantic segments of 3D shapes without any direct supervision, based only on using \textbf{linguistic} descriptions comparing shapes. 
    
    \item While Transformers has been used to discover semantic parts in 2D images, we are the first to segment \textbf{3D} shapes using Transformer attention.
    
    \item Importantly, we do NOT argue that 3D parts just emerge from Transformer-based learning (as done by Caron \emph{et al.}~\citecaron{}, the work mentioned by \textbf{\RTwo}). In fact, our analysis shows that a straightforward adaptation of Transformers to our 3D setting does NOT provide meaningful 3D segmentation -- but our \textbf{careful network design} can accomplish this task.
    
    \item We demonstrate the generalizability of our network to out-of-distribution categories for the more demanding \textbf{segmentation} task, not for the easier target discrimination task in reference games presented in ShapeGlot.
\end{enumerate}
\vspace{-0.5\baselineskip}

\noindent More details are given below.

\vspace{-\baselineskip}
\paragraph{(1)} We appreciate the reviewers finding that we propose a ``very interesting'' and ``novel'' application (\ROne) --- segmenting 3D shapes using natural language, which ``addresses the long-standing problem of reducing 3D annotations'' (\RThree). While there is previous work relating linguistic descriptions with 3D shapes, semantic part segmentation based only on language descriptions hasn't been attempted. For the first time, we introduce this novel problem, propose a method, and demonstrate ``impressive results'' (\RThree) with comprehensive analyses based on ``lots of experimental results'' (\RTwo).

\vspace{-\baselineskip}
\paragraph{(2) and (3)} 
While Caron \emph{et al.}~\citecaron{} observe the emergence of semantic segments in 2D images when training a Vision Transformer (ViT), \textbf{we argue that just plugging in Transformer to a 3D network does not produce meaningful segmentation results.} See rows 3 and 11 in Table 2 of our paper. In particular, when the raw point cloud is fed to the network instead of the super-segments, or when the global feature is concatenated to the point features as done in PointNet, the average mIoU goes down to \textbf{22.5} and \textbf{30.3} in the PN-Aware case.  In contrast, our method uses super-segments and does not use global features. It also normalizes the query, key and value vectors (which is not commonly done in Transformers). Additionally, it uses a double softmax in a particular order, along with a cross entropy loss. All of these implementation decisions lead to the much superior mIOU of \textbf{79.4} (row 2).

% As well as using super-segments and removing global features, when also normalizing the query, key, and value vectors (which is not common in Transformers) and using a double softmax in proper order and the cross-entropy loss, the average mIoU can be increased to \textbf{79.4} (row 2).

\vspace{-\baselineskip}
\paragraph{(4)} 
While ShapeGlot demonstrates out-of-distribution generalizability for the \textbf{classification task} of selecting the target shape in a language reference game, we show generalizability on a much \textbf{more challenging and granular} task -- segmenting 3D shapes via attention. To the best of our knowledge, our network is the first to be designed for this task. Thus, the generalizability we show is not trivial.


\vspace{-\baselineskip}
\paragraph{Results with PartNet~\citepartnet{} Parts [\RThree]}
In our experiments, we used the four part classes (back, seat, leg, arm) of Chair in ShapeNet to match the majority of part names used in CiC utterances, not to limit the number of the parts. To experiment with more parts, we would require a new reference game dataset that contains new part names in descriptions.

Here, we demonstrate experimental results with \emph{synthetic} reference games created using the parts in PartNet~\citepartnet{}. We tested with two categories separately: Chair and Table. Among the parts in \emph{level 2} of the PartNet hierarchy, we randomly sample one of them and synthesize an utterance with template sentences (shown in Figure~\ref{fig:partnet}) indicating the existence or absence of a part. Given the utterance, target and distractor shapes are also randomly sampled based on part existence. Part classes which are present or absent in less than 10\% of shapes are excluded. %from the synthetic utterances
Figure~\ref{fig:partnet} illustrates some qualitative results. Finer-grained parts such as frame, support, and stretcher are accurately discovered. Table below also shows the average mIoUs, which are comparable with the \emph{supervised} segmentation result using PointNet, shown in Table 3 of PartNet~\citepartnet{}.
% The average mIoUs for both PN-Agnostic and PN-Aware network trained on this dataset are \textbf{35.3} and \textbf{32.7} respectively, which are comparable with the \emph{supervised} segmentation result using PointNet (\textbf{38.2}), shown in Table 2 of PartNet.

%%%%%%%%
% \vspace{0.5\baselineskip}
% {
% \centering
% \footnotesize
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \begin{tabularx}{\linewidth}{Y|YYY}
% \toprule
% Category & PN-Agnostic & PN-Aware & Supervised~\citepartnet{} \\
% \midrule
% Chair & 35.3 & 32.7 & \textbf{38.2} \\
% Table & \textbf{44.0} & 33.7 & 34.3 \\
% \bottomrule
% \end{tabularx}
% }
\input{tables/table_partnet_results}
%%%%%%%%

\vspace{-\baselineskip}
\paragraph{Low Arm IoU [\ROne]}
%Arm is the only \emph{optional} part, and many chairs do not have the part. If arm does not exist, even when a \textit{single} point is classified as arm, the IoU becomes 0. Due to this non-smooth metric definition, it is harder to achieve a high IoU for arm.
Arm is the only \emph{optional} part, and many chairs do not have the part. If arm does not exist, even when a single point is
classified as arm, IoU becomes zero. Hence, it is more challenging to achieve high IoU for arm compared to the other parts.

\vspace{-0.5\baselineskip}
{\footnotesize
\paragraph{References}\hfill\\
\noindent[1] M. Caron \emph{et al.}, Emerging Properties in Self-Supervised Vision Transformers, In ICCV, 2021.\\
\noindent[2] K. Mo \emph{et al.}, PartNet: A Large-scale Benchmark for Fine-grained and Hierarchical Part-level 3D Object Understanding, In CVPR, 2019.\\
}


==> rebuttal/review_juil.tex <==
\section{Review Summary}
\paragraph{Reviewer 1}
WA. 
\begin{enumerate}
    \item Low arm IoUs of PN-AG and PN-AW (Id 1 and 2 in table 2.)
\end{enumerate}

\paragraph{Reviewer 2}
WR.
\begin{enumerate}
    \item claimed that the architecture has just changed from CNN in Shapeglot to Transformer. 
    \item Some contributions that authors claim are not from their method but from Transformer architecture itself or the contribution already claimed in Shapeglot.
    \item Generalization to OoD has already been shown in Shapeglot.
    \item .[2] has already shown the weakly-supervised segmentation ability of ViT in the image domain.
\end{enumerate}
[2] M.Caron, Emerging Properties in Self-Supervised Vision Transformers, ICCV 2021
\paragraph{Reviewer 3}
WA.
\begin{enumerate}
    \item Wondering the results on more complex dataset. (e.g., PartNet)
\end{enumerate}


%%%%%%%%%%%%%%%%

\section{Rebuttal}

\paragraph{[R2] ``Some contributions are from Transformer architecture itself or Shapeglot."}
\begin{itemize}
    \item \textbf{Different generalization ability}
    The generalization ability shown in Partglot and Shapeglot represents a completely different meaning. Shapeglot focused on understanding and differentiating the structures of unseen categories, i.e., classification, but we have demonstrated that the learned relation between semantic parts and referential language has a capacity of generalizing ``part information" to unseen categories' parts. Not only did we take care of a different task, classification and part segmentation, but we showed that even the parts that are differently labeled across categories can be generalized by relation between compositions and language, e.g., Chair seat and Table top entail a compositionally similar meaning, which wasn't  shown in Shapeglot. 
    \item \textbf{Initiating to utilize Transformer in part segmentation by language.}
    Our method and domain completely differs with [2]. We haven't just applied existing transformer architectures or methods related to that on 3D part segmentation, but we have elaborated the network with various details and introduced how language can successfully guide the network to learn 3D part segmentation with barely given geometry priors. Table 2 presents a plenty of our design choices and their importance. Recap of details is below.
    \begin{enumerate}
        \item \textbf{Various design details}
        We have experimentally demonstrated that our design details, including normalizing features, removing the global feature and the order of applying softmaxes, are crucial for enabling the attention to precisely highlight the semantic parts. Within a very limited provided supervision, we also further improved mIoUs by a regularization loss that successfully prevent attention maps from overlapping.
        \item \textbf{}
    \end{enumerate}
    
\end{itemize}

\paragraph{[R3] ``Can the model perform in more fine-grained parts? e.g., PartNet"}
Chair: back, seat, leg, arm (+head, footrest, wheel)
Lamp: (+power\_cord, 
% \paragraph{Reviewer 1}
% \paragraph{Reviewer 2}
% 
% \begin{enumerate}
%     \item \& 2. As the reviewer 3 mentioned, we have already presented extensive ablation studies to demonstrate each our specific design choice plays an important role to achieve superb mIoUs (specifically average 79\%). The table 2 shows that the network fails to obtain meaningful results if any our specific design choice is removed. Thus, we argue that we haven't just incorporated Transformer into Shapeglot, rather we have elaborated the network to utilize supervision from language to facilitate 3D part annotations. Recap of design choices is below.
%     \begin{itemize}
%         \item \textbf{The importance of design details} 
%         We have experimentally demonstrated that specific design details, including normalizing the features, removing the global feature and the order of softmaxes, are crucial for enabling the attention to precisely highlight the semantic parts.
%         \item \textbf{Providing various setups}
%         We have considered two setups, whether the set of part names is given in advance or not, and developed a pipeline to further leverage supervision from the part names.  
%         \item \textbf{A novel regularization}
%         We have introduced a regularization loss based on cross entropy. Within limited supervisions, the regularization has succeeded to prevent attention maps from overlapping, which results in increasing IoUs overall.
%         \item \textbf{Finding the effect of granularity}
%         We have shown the importance of using super-segments, not just directly applying attention mechanism on point clouds.
%     \end{itemize}
    
%     \item The generalization ability shown in Partglot and Shapeglot represents a completely different meaning. Shapeglot focused on understanding and differentiating the structures of unseen categories, but we have demonstrated that ours can generalize ``part" information to other categories' semantically corresponding parts. 
%     \item 
%     \begin{itemize}
%         \item \textbf{difference between ours and existing ViTs.}
%         Even though [2] showed ViT had some ability to weakly supervised segmentation, ours method completely differs and the domain as well. We haven't just applied existing ViTs in the image domain on 3d part segmentation, but built the very carefully designed network. Table 2 shows applying simply Transformer on part segmentation fails. 
%         \item \textbf{Novel method of leveraging language for part segmentation}
%         To our best knowledge, there has been no work as to leveraging language supervision for 3D part segmentation. Despite initiating the novel method, we have enough shown very attractive results and the advantage from language, generalizing part information on Out-of-Distribution categories.
%         \item \textbf{Drawbacks of using images for part segmentation}
%         When we consider 2D images as input, it cannot handle occluded parts. Our network doesn't require further rendering or like that pipeline.
%     \end{itemize}
%     \item (+) Our network relatively requires low cost. (DINO [2] takes 16-GPU over 3 days to train, but ours is trained within 3~4hours on a 3090.)

% \end{enumerate}

% \paragraph{Reviewer 3}
% \subparagraph{PartNet Experiment}


==> tables/table_granularity.tex <==
\begin{table}[h!]
\centering
\caption{Super-segment statistics.}
{\footnotesize
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{\linewidth}{>{\centering}m{1.3cm}|>{\centering}m{1.3cm}|YYYYY}
\toprule
$N$ & Mean \# Super-Segs & Back & Seat & Leg & Arm & Avg \\
\midrule
512 \textbf{(Ours)} & 18.4 & 84.9 & 83.6 & 78.9 & 70.4 & 79.4 \\
256 & 20.2 & & & & &\\
128 & 24.4 & & & & &\\ 
64 & 36.4 & 53.4 & 21.5 & 63.7 & 36.0 & 43.7 \\ 
32 & 65.6 & 57.2 & 5.4 & 60.2 & 11.9 & 33.7 \\ 
16 & 128.2 & & & & &\\
\bottomrule
\end{tabularx}
\centering 
}
\label{tbl:data_stats}
\end{table}
